Nonuniform Reductions and NP-Completeness

Nonuniformity is a central concept in computational complexity with powerful connections to circuit complexity and randomness. Nonuniform reductions have been used to study the isomorphism conjecture for NP and completeness for larger complexity classes. We study the power of nonuniform reductions for NP-completeness, obtaining both separations and upper bounds for nonuniform completeness vs uniform completeness in NP. Under various hypotheses, we obtain the following separations: 1. There is a set complete for NP under nonuniform many-one reductions, but not under uniform many-one reductions. This is true even with a single bit of nonuniform advice. 2. There is a set complete for NP under nonuniform many-one reductions with polynomial-size advice, but not under uniform Turing reductions. That is, polynomial nonuniformity is stronger than a polynomial number of queries. 3. For any fixed polynomial p(n), there is a set complete for NP under uniform 2-truth-table reductions, but not under nonuniform many-one reductions that use p(n) advice. That is, giving a uniform reduction a second query makes it more powerful than a nonuniform reduction with fixed polynomial advice. 4. There is a set complete for NP under nonuniform many-one reductions with polynomial advice, but not under nonuniform many-one reductions with logarithmic advice. This hierarchy theorem also holds for other reducibilities, such as truth-table and Turing. We also consider uniform upper bounds on nonuniform completeness. Hirahara (2015) showed that unconditionally every set that is complete for NP under nonuniform truth-table reductions that use logarithmic advice is also uniformly Turing-complete. We show that under a derandomization hypothesis, the same statement for truth-table reductions and truth-table completeness also holds.

==> 2-separation.tex <==
\begin{theorem}
If $\mu_p (\NP) \neq 0$ then there exists a set $A \in \NP$ that is $\le_{2-tt}^p$-complete but is not $\le_m^{P/1}$-complete.
\end{theorem}
\begin{proof}
Let $R \in \NP \cap \coNP$ be $p$-random, and define $A = 0(R \cap \SAT) \cup 1(\bar{R} \cap \SAT)$, where $\bar{R}$ is $R$'s complement. Then $A \in \NP$ by closure properties of $\NP$, and $\SAT \le_{2-tt}^p$ since $x \in \SAT \leftrightarrow (0x \in A \vee 1x \in A)$. Therefore $A$ is $\le{2-tt}^p$-complete in $\NP$. We will show that $A$ is not $\le_m^{P/1}$-complete. To get a contradiction, assume that $R \le_m^{P/1} A$ via $f \in PF$ and $h : \N \rightarrow \{0 , 1 \}$. In other words, 
$(\forall x)\; R[x] = A [ f\big( x , h(|x|) \big)]$. In many cases in the rest of the proof we need to eliminate the prefix of $0$ or $1$ from queries to $A$, therefore we define a function $v : \{ 0 , 1 \}^* \rightarrow \{0 , 1 \}^*$ as $v(0x) = v(1x) = x$ for every string $x$. Bases on the value of $f(z , 0)$ and $f(z , 1) $ in comparison with the input string $z$ there are $9$ possible cases as follows:
\begin{enumerate}
\item $v \big( f ( z , 0) \big) = v \big( f ( z , 1) \big) = z $ 
\item $v \big( f ( z , 0) \big) = z $ and $v \big( f ( z , 1) \big) < z $
\item $v \big( f ( z , 0) \big) < z $ and $v \big( f ( z , 1) \big) = z $
\item $v \big( f ( z , 0) \big) = z $ and $v \big( f ( z , 1) \big) > z$
\item $v \big( f ( z , 0) \big) > z $ and $v \big( f ( z , 1) \big) = z $
\item $v \big( f ( z , 0) \big) < z $ and $v \big( f ( z , 1) \big) < z $
\item $v \big( f ( z , 0) \big) > z $ and $v \big( f ( z , 1) \big) < z $
\item $v \big( f ( z , 0) \big) < z $ and $v \big( f ( z , 1) \big) > z $
\item $v \big( f ( z , 0) \big) > z $ and $v \big( f ( z , 1) \big) > z $
\end{enumerate} 
We will show that none of these cases can happen for infinitely many $z$'s where $z \notin \SAT$.
\begin{claim}\label{firstclaim}
There cannot be infinitely many $z$'s such that $z \notin \SAT$ and $z$ satisfies the first condition.
\end{claim}
\begin{proof}
Assume there are infinitely many $z$'s such that $z \notin \SAT$ and $v \big( f ( z , 0) \big) = v \big( f ( z , 1) \big) = z $. This implies that for each one of these $z$'s we have $A[f(z , 0)] = A[f(z , 1)] = 0$. As a result, $R[z] = 0$ no matter what the advice is. Define a martingale that on input $z$ first computes $\SAT[z]$. If $z \notin \SAT$ then it computes $f(z , 0)$ and $f(z , 1)$. If $v \big( f(z , 0) \big) = v \big( f(z , 1) \big)$ then it bets all of the capital on $R[z] = 0$. In any other case, our martingale does not bet on $z$. It is easy to see that this is a polynomial-time martingale, and it succeeds on $R$. As a result \rm{Claim 1} holds.
\end{proof}

In the rest of the proof we will assume that the first case does not happen if $z \notin \SAT$. 
\begin{claim}\label{secondclaim}
Let $A_n = \{ z \; | \; z \notin \SAT, \;  |z| = n, \; \text{and one of the first eight cases occurs for z} \}$. Then $(\forall^{\infty} n) \; |A_n| \le n$. In other words, for almost every $n$ there are at most $n$ strings $z_1,..., z_n$ of length $n$ such that 
$v \big( f(z_i , 0) \big) \le z_i$ or $v \big( f(z_i , 1) \big) \le z_i$.
\end{claim}
\begin{proof}
Assume \rm{Claim 2} does not hold. Then there exists infinitely many $n$'s such that
$|A_n| \geq n+1$. We use this to define a polynomial-time martingale that succeeds on $R$. For each length $n$ our martingale first checks if $|A_n| \geq n+1$. This can be done in $2^{3n}$ steps. We do not bet if $ |A_n| < n+1$. On the other hand, if $|A_n| \geq n+1$ then we bet on the first and possibly one more string in $A_n$. Let $z_1,...,z_{n+1}$ be the first $n+1$ strings in $A_n$. First we compute $f(z_1 , 0)$ and $f(z_1 , 1)$. If case $2$, $3$, $4$, $6$ or $8$ happens then we bet $2/3$ of the capital on $R[z_1]$ being equal to  $A[f(z_1 , 0)]$. On the other hand, if case $5$ or $7$ occurs then we bet $2/3$ of the capital on $R[z_1]$ being equal to $A[f(z_1 , 1)]$. Basically we are giving more weight to the possibility that the correct advice  creates a shorter query. If we win the capital will be multiplied by $4/3$, and we will not bet on any other string of length $n$. On the contrary, if we lose the capital will be reduced by a factor of $2/3$, but we will know the correct advice for length $n$. We will use this to make another bet as follows. Assume the correct advice for length $n$ is $i$. First compute $f(z_2 , i),..., f(z_{n+1} , i)$. If there exists $2 \le j \le n+1$ such that $v \big( f(z_j , i) \big) \le z_j$ then we compute $A[f(z_j , i)]$ in $2^{2|z_j|}$ steps. We know that $R[z_j] = A[f(z_j , i)]$ therefore we can double our capital by betting on $z_j$, and end up with $2 * 2/3 = 4/3$ of the original capital. On the other hand, assume that for every $2 \le j \le n+1$ we have $v \big( f(v_j , i) \big) > z_j$. This means $R[z_j] = \tilde{R} \cap \SAT[z_j^1]$ for some $z_j^1 > z_j$ (Here $\tilde{R}$ stands for $R$ or $\bar{R}$ depending on whether the first bit of $f (z_j , i)$ is $0$ or $1$ respectively. Note the assumption that $R$ is $p$-random implies that for at least $2/3$ of the $n$'s there exists a $z_j$ among $z_2,...,z_{n+1}$ such that $z_j \in R$. \textbf{Do we need to prove this?} 
In these cases we know that $\tilde{R}[z_j^1] = 1$. We use this fact to bet on $z_j^1$ and double the capital. As a result, we will end up with $4/3$ of the original capital in these cases. Note that in the cases that such $z_j$ does not exist the capital will be multiplied by $2/3$, but this happens at most $1/3$ of the times. Hence the capital will be multiplied by at least $(2/3)^m * (4/3)^{2m} = (32/27)^m$ where $m = n/3$. This shows that there exists a polynomial-time martingale that succeeds on $R$, which is a contradiction. Therefore \rm{Claim 2} holds. 
\end{proof}

\begin{claim}
If there are infinitely many $n$'s such that for each one of them there are three strings of length $n$, $z_1$, $z_2$, and $z_3$, such that $v \big( f(z_1 , 0) \big) = v \big( f(z_2 , 1) \big) = v \big( f(z_3 , 1) \big) = y$ for some $y > z_1,z_2$, and $z_3$ then $R$ is not $p$-random.
\end{claim}
\begin{proof}
Assume the premise of the claim does not hold. W.L.O.G assume that $f(z_1 , 0) = 0y$ for some string $y$. We will consider three cases:
\begin{enumerate}
\item $f(z_2 , 1) = 0y$. Since the correct advice is either $0$ or $1$ we have $R \cap \SAT[y] = R[z_1]$ or $R[z_2]$. If this happens i.o. then by $p$-randomness of $R$ there must be infinitely many cases where $R[z_1] = R[z_2] = 1$. \textbf{Does this need a proof?}
This implies $R[y] = 1$. As a result, there is a martingale that succeeds on $R$, which is a contradiction.
\item $f(z_2 , 1) = f(z_3 , 1) = 1y$. W.L.O.G. assume that $z_3 > z_2$. If $1$ is the right advice then we will have $R[z_2] = R[z_3]$. First we assume this is the case, and bet $2/3$ of the capital on $R[z_3]$ being equal to $R[z_2]$. If we are right the capital will be multiplied by $4/3$. On the other hand, if $R[z_3] \neq R[z_2]$ then we will end up with $2/3$ of the original capital, but we will know that the correct advice is $0$. Therefore $R[z_1] = R \cap \SAT[y]$. For the cases where $R[z_1] = 1$ this implies that $R[y] = 1$. We can use this to double the capital and end up with $4/3$ of the original capital. \textbf{??}
\item $f(z_2 , 1) = 1y$ and $f(z_3 , 1) = 0y$. Similar to the first case.
\end{enumerate}
\end{proof}
Let $B = \{z \; | \; z \notin \SAT ,\; |z| = n,\;  v \big( f(z , 0) \big) > z, \; and \; 
v \big( f(z , 1) \big) > z \}$. \rm{Claim 2} and randomness of $R$ implies that there must be infinitely many $n$'s such that there are three strings of length $n$ in $B \cap R$. We define a martingale that succeeds on $R$ using these strings. Let $z_1$, $z_2$, and $z_3$ be such three strings of length $n$, and W.L.O.G. assume that $v \big( f(z_1 , 0) \big)$ is the smallest string among $v \big( f(z_i , j) \big)$'s where $1 \le i \le 3$ and $j = 0$ or $1$. First we assume that $0$ is the correct advice. In other words, we assume that $R[z_1] = \tilde{R} \cap \SAT[v \big( f(z_1 , 0) \big)]$ where $\tilde{R}$ is either $R$ or $\bar{R}$ depending on whether the first bit of $f(z_1 , 0)$ is $0$ or $1$. This implies that $v \big( f(z_1 , 0) \big) \in \tilde{R}$. We bet $2/3$ of the capital on 
$v \big( f(z_1 , 0) \big) \in \tilde{R}$. If we win we do not bet on any string that of length less that or equal to $|v \big( f(z_1 , 0) \big)|$. On the other hand, if $\tilde{R}[v \big( f(z_1 , 0) \big)] = 0$ then know that the correct advice is $1$. As a result, we will know that $R[z_2] = \tilde{R} \cap \SAT[v \big( f(z_2 , 1) \big) ]$. Therefore $\tilde{R}[v \big( f(z_2 , 1) ] = 1$. We use this to bet on $v \big( f(z_2 , 1) \big)$, and double the capital. Note that the only problem with this strategy is when 
 $v \big( f(z_2 , 1) \big)$ is the same as  $v \big( f(z_1 , 0) \big)$. But by \rm {Claim 3} we know that at least one of  $v \big( f(z_2 , 1) \big)$ and  $v \big( f(z_3 , 1) \big)$ must be different from $v \big( f(z_1 , 0) \big)$, which completes the proof.
\end{proof}


==> conclusion.tex <==
\section{Conclusion}


